Serpens: A High Bandwidth Memory Based Accelerator for General-Purpose Sparse Matrix-Vector Multiplication

Sparse matrix-vector multiplication (SpMV) multiplies a sparse matrix with a dense vector. SpMV plays a crucial role in many applications, from graph analytics to deep learning. The random memory accesses of the sparse matrix make accelerator design challenging. However, high bandwidth memory (HBM) based FPGAs are a good fit for designing accelerators for SpMV. In this paper, we present Serpens, an HBM based accelerator for general-purpose SpMV.Serpens features (1) a general-purpose design, (2) memory-centric processing engines, and (3) index coalescing to support the efficient processing of arbitrary SpMVs. From the evaluation of twelve large-size matrices, Serpens is 1.91x and 1.76x better in terms of geomean throughput than the latest accelerators GraphLiLy and Sextans, respectively. We also evaluate 2,519 SuiteSparse matrices, and Serpens achieves 2.10x higher throughput than a K80 GPU. For the energy/bandwidth efficiency, Serpens is 1.71x/1.99x, 1.90x/2.69x, and 6.25x/4.06x better compared with GraphLily, Sextans, and K80, respectively. After scaling up to 24 HBM channels, Serpens achieves up to 60.55~GFLOP/s (30,204~MTEPS) and up to 3.79x over GraphLily. The code is available at https://github.com/UCLA-VAST/Serpens.

==> texfiles/table_compare.tex <==
\begin{table*}[tb]
\caption{Comparison with related sparse and dense accelerators.}
  \label{table:comparison}
  \centering
  \vspace{-6pt}
  \begin{threeparttable}
  \begin{tabular}{ccccccccc}
    \hline
    & \textbf{Kernels} & \textbf{Mat. NNZ} & \textbf{Prob. Size} &
    \textbf{Throughput} & \textbf{FPGA} & \textbf{ASIC} & \textbf{Real Exe.}& \textbf{1-for-all}\\
    \hline
    %\hline
    T2S-Tensor \cite{srivastava2019t2s} & Dense MM, MV, etc\tnote{1} & $2\times10^3$ & - &
    738 GFLOP/s & \textbf{Yes} & No & \textbf{Yes} & No \\
    
    %\hline
    AutoSA \cite{wang2021autosa} & Dense MM, etc\tnote{1} & $4\times10^6$ & $7\times10^9$ &
    950 GFLOP/s & \textbf{Yes} & No & \textbf{Yes} & No \\
    
    
    %\hline
    \cite{fowers2014high} & SpMV & $5\times10^6$ & $<1\times10^7$ &
    3.9 GFLOP/s & \textbf{Yes} & No & \textbf{Yes} & No \\
    
    
    %\hline
    Spaghetti \cite{hojabr2021spaghetti} & SpGEMM & $1.6\times10^7$ & - &
    27 GFLOP/s & \textbf{Yes} & No & \textbf{Yes} & No \\
    
    
    
    

    
    %\hline
    Tensaurus \cite{srivastava2020tensaurus} & SpMV, SpMM, etc\tnote{2} & $4.2\times10^6$ & - &
    512 GFLOP/s\tnote{3} & No & \textbf{Yes} & No & No \\
    
    %\hline
    ExTensor \cite{hegde2019extensor} & SpMM, SpGEMM, etc\tnote{2} & $6\times10^6$ & - &
    64 GFLOP/s & No & \textbf{Yes} & No & No \\
    
    %\hline
    SIGMA \cite{qin2020sigma} & SpGEMM & - & - &
    - & No & \textbf{Yes} & No & No \\
    
    
    
    
    
    %\hline
    SpArch \cite{zhang2020sparch} & SpGEMM & $1.65\times10^7$ & - &
    10.4 GFLOP/s & No & \textbf{Yes} & No & No \\
    
    
    
    
    
    %\hline
    OuterSPACE \cite{pal2018outerspace} & SpGEMM & $1.65\times10^7$ & - &
    2.9 GFLOP/s & No & \textbf{Yes} & No & No \\
    
    
    %\hline
    SpaceA \cite{xie2021spacea} & SpMV & $1.4\times10^7$ & $1.43\times10^7$ &
    - & No & \textbf{Yes} & No & No \\
    
    %\hline
    \sextansFPGA & SpMM & $3.7\times10^7$ & $3\times10^{10}$ &
    181.1 GFLOP/s & \textbf{Yes} & No & \textbf{Yes} & \textbf{Yes} \\
    
    %\hline
    \sextansASIC & SpMM & $3.7\times10^7$ & $3\times10^{10}$ &
    1281 GFLOP/s & No & \textbf{Yes} & No & \textbf{Yes} \\
    \hline
  \end{tabular}
  
  
  \begin{tablenotes}
        \footnotesize
        \item[1] Other dense tensor kernels such as TTMc, MTTKRP are also supported. $^2$ Other dense tensor kernels such as sparse TTM, sparse TTV are also supported.
        \item[3] 512 GFLOP/s is achieved on dense multiplication, and the throughput of sparse multiplication is lower.  
      \end{tablenotes}
    \end{threeparttable}
  
\end{table*}
